Learning Good Interventions in Causal Graphs via Covering

We study the causal bandit problem that entails identifying a near-optimal intervention from a specified set $A$ of (possibly non-atomic) interventions over a given causal graph. Here, an optimal intervention in ${A}$ is one that maximizes the expected value for a designated reward variable in the graph, and we use the standard notion of simple regret to quantify near optimality. Considering Bernoulli random variables and for causal graphs on $N$ vertices with constant in-degree, prior work has achieved a worst case guarantee of $\widetilde{O} (N/\sqrt{T})$ for simple regret. The current work utilizes the idea of covering interventions (which are not necessarily contained within ${A}$) and establishes a simple regret guarantee of $\widetilde{O}(\sqrt{N/T})$. Notably, and in contrast to prior work, our simple regret bound depends only on explicit parameters of the problem instance. We also go beyond prior work and achieve a simple regret guarantee for causal graphs with unobserved variables. Further, we perform experiments to show improvements over baselines in this setting.

==> Include/regret-analysis-observable.tex <==

\subsection{Regret Analysis}
\label{section:regret-analysis}

We first state a standard concentration bound which will be used in the analysis. 
\begin{lemma} [Hoeffding's Inequality] \label{lem:hoeff}
Let $Z_1, \ldots, Z_n$ be independent bounded random variables with $Z_i \in [a_i, b_i]$, for all $i \in [n]$. Then, %, where $-\infty<a_i \leq b_i<\infty$
$$
\mathbb{P}\left( \left| \sum_{i=1}^n\left(Z_i-\mathbb{E}\left[Z_i\right]\right) \right|  \geq \varepsilon \right ) \leq 2 \exp \left(-\frac{2  \varepsilon ^2}{\sum_{i=1}^n (b_i-a_i)^2}\right),
$$
for all $\varepsilon \geq 0$.
\end{lemma}

For any intervention $A \in \cA$, the estimate $\muh(A)$ can be expressed as 
\begin{align*}
	\widehat{\mu} \left(A \right) & = \sum_{\zd \in Z(A)} \prod_{ i \in \cV(A)} \left (\cP{\zd_i}{\zd_{\pa(i)}}{} +  \Delta \cP{\zd_i}{\zd_{\pa(i)}}{}\right )                                                       \\
	                              & = \mu (A) + \sum_{\zd \in Z(A)} \left ( \sum_{ i \in \cV (A)} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \prod_{ j \in \cV(A), j\neq i}  \cP{\zd_j}{\zd_{\pa(j)}}{} \ + \ \mathcal{L}_\zd \right ) 		\tag{expanding the product}	  
\end{align*}
Here, $\mathcal{L}_\zd$ represents all the product entries in the expansion that include more than one error term ( $\Delta \cP{}{}{}$). Specifically, 
\begin{align}
	\mathcal{L}_\zd  = \sum_{k = 2}^{|\cV (A)|} \sum_{\substack{U \subseteq \cV(A) \\ |U| = k}} \left(\prod_{i \in U } \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \right) \left(\prod_{j \in \cV(A) \setminus U} \cP{\zd_j}{\zd_{\pa(j)}}{} \right) \label{eqn:Lz}
\end{align}
We further write $\mathcal{H}_\zd$ to represent the sum of the entries with a single error term:
\begin{align}
	\mathcal{H}_\zd \coloneqq  \left ( \sum_{ i \in \cV (A)} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \prod_{ j \in \cV(A), j\neq i}  \cP{\zd_j}{\zd_{\pa(j)}}{} \right) \label{eqn:Hz}
\end{align}
Hence,%\footnote{Note that both $\mathcal{H}$ and $\mathcal{L}$ depend on an assignment $\zd \in Z(A)$. We suppress this dependence for ease of notation.}  
\begin{align*}
    \muh(A) - \mu(A) = \sum_{\zd \in Z(A)} \left( \mathcal{H}_\zd + \mathcal{L}_\zd
    \right)
\end{align*}
We will establish upper bounds on the sums of $\mathcal{L}_\zd$s and $\mathcal{H}_\zd$s and in Lemma \ref{lem:l-bound} and Lemma \ref{lem:h-bound}, respectively. These lemmas show that the sum of the $\mathcal{H}$ terms dominates the sum of $\mathcal{L}$ terms. Furthermore, these bounds imply that the estimated reward  $\muh(A)$ is sufficiently close to the true expected reward $\mu(A)$ for each intervention $A \in \cA$.  

\begin{lemma} \label{lem:er_bound}
For estimates obtained via a covering intervention set $\cI$, as in Algorithm \ref{algo: main algo fully obs setting}, write $\mathcal{E}$ to denote the event that $|\Delta \cP{\zd_i}{\zd_{\pa(i)}}{}| \leq \sqrt{\frac{|\cI| (d+ \log{(NT)})}{T}}$ for all vertices $i \in \cV$. Then, $\Pr\{ \mathcal{E}\} \geq \left( 1-\frac{2}{T} \right)$.
%	\begin{align*}
%		|\Delta \cP{\zd_i}{\zd_{\pa(i)}}{}| \leq \sqrt{\frac{|\cI| (d+ \log{(NT)})}{T}} & \qquad \text{for all $i \in \cV$.}
%	\end{align*}
\end{lemma}
\begin{proof}
Since $\cI$ is a covering intervention set, for each conditional distribution $\cP{\zd_i } {\zd_{\pa(i)}}{}$, we have at least $\frac{T}{|\cI|}$ independent samples. Now, we invoke Lemma \ref{lem:hoeff}, with $\varepsilon = \sqrt{\frac{|\cI| \log{(2^d NT)}}{T}}$, and apply the union bound over all $i \in [N]$ and all assignments to $\pa(i)$. This gives us the desired probability bound. \
\end{proof}
\begin{lemma}\label{lem:l-bound}
For estimates obtained via a covering intervention set $\cI$, as in Algorithm \ref{algo: main algo fully obs setting}, the following event holds with probability at least $\left( 1-\frac{2}{T} \right)$:
\begin{align*}
\sum_{\zd \in Z(A)} \left| \mathcal{L}_\zd  \right| \leq 4(N\eta)^2 \qquad \text{for all $A \in \cA$.}
\end{align*}
Here, parameter $\eta = \sqrt{\frac{|\cI| (d+\log{(NT)})}{T}} $ and $T$ is moderately large $T$.
\end{lemma}
\begin{proof}
    We will use the fact that each error term in $\mathcal{L}_\zd$ satisfies the bound stated in Lemma \ref{lem:er_bound}. Moreover, we utilize the graph structure to marginalize variables that do not appear in an expansion of $\mathcal{L}_\zd$.
	\begin{align*}
		\sum_{\zd \in Z(A)} |\mathcal{L}_\zd | \leq \sum_{\zd \in Z (A)} \sum_{k = 2}^{|\cV (A)|} \sum_{\substack{U \subseteq \cV(A) \\ |U| = k \ \ }} \left(\prod_{i \in U }  \left| \Delta \cP{\zd_i}{\zd_{\pa(i)}}{}\right| \right) \left(\prod_{j \in \cV(A) \setminus U} \cP{\zd_j}{\zd_{\pa(j)}}{} \right)\\
		= \sum_{k = 2}^{|\cV (A)|} \sum_{\zd \in Z (A)}  \sum_{\substack{U \subseteq \cV(A) \\ |U| = k \ \ }} \left(\prod_{i \in U } \left |\Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \right |  \right) \left(\prod_{j \in \cV(A) \setminus U} \cP{\zd_j}{\zd_{\pa(j)}}{} \right).
	\end{align*}

	First, we upper bound each term considered in the outer-most sum. Towards this, let $U =\{V_{x_1}, V_{x_2}, \ldots, V_{x_k}\}$ to be a subset of vertices that appears in the inner sum. Here, $x_1 < x_2 < \ldots < x_k$ and, as mentioned previously, the indexing of the vertices respects a topological ordering over the causal graph. In the derivation below, we will split the sum into $k$ parts, $\sum_{\zd_{[1:x_1]}} \sum_{\zd_{(x_1:x_2]}} \ldots \sum_{\zd_{(x_k:N]}} $, and individually bound the marginalized probability distribution.
 %Let $S = \{x_1, x_2 \ldots , x_k \}$ where  $x_i$ denotes the index in set $\cV(A)$ and let $\cV_U(A) = \cV(A) \cap  U$ for some $U \subset \cV$.
	\begin{align}
		&\sum_{\zd \in Z (A)}  \sum_{\substack{U \subseteq \cV(A) \\ |U| = k}} \left(\prod_{i \in U } \left |\Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \right |  \right) \left(\prod_{j \in \cV(A) \setminus U} \cP{\zd_j}{\zd_{\pa(j)}}{} \right) \nonumber\\ 
		&\leq \sum_{\substack{U \subseteq \cV(A) \\ |U| = k}} \sum_{\zd \in Z (A)} \eta^k   \left(\prod_{j \in \cV(A) \setminus U} \cP{\zd_j}{\zd_{\pa(j)}}{} \right) \nonumber \tag{via Lemma \ref{lem:er_bound}, $\left|\Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \right| \leq \eta$ }\\ 
		&= \sum_{\substack{U \subseteq \cV(A) \\ |U| = k}} \eta ^k 
		\sum_{\zd_{[1: \x_1]} \in Z_{[1: \x_1]}(A)} 
		\left(\prod_{j_1 \in  \cV_{[1:x_1) }(A) } \cP{\zd_{j_1}}{\zd_{\pa(j_1)}}{} \right) \sum_{\zd_{(x_1: \x_2]} \in Z_{(x_1: x_2]}(A)} \left(\prod_{j_2 \in  \cV_{(x_1:x_2) }(A) } \cP{\zd_{j_2}}{\zd_{\pa(j_2)}}{} \right)  \nonumber
		\ldots
		 \\& \sum_{\zd\in Z_{(x_i: x_{i+1}]}(A)} \left(\prod_{j_i \in \cV_{(x_i:x_{i+1}) }(A) } \cP{\zd_{j_i}}{\zd_{\pa(j_i)}}{} \right) \ldots \sum_{\zd_{(x_k : N ]} \in Z_{(x_k: N]}(A)} \left(\prod_{j_k \in \cV_{(x_k:N] }(A) } \cP{\zd_{j_k}}{\zd_{\pa(j_k)}}{} \right) \label{eqn:sec}
	\end{align}

	The last term in the above expression can be bounded as follows 
	\begin{align*}
		\sum_{\zd_{(x_k: N]} \in Z_{(x_k: N]}(A)} \left(\prod_{j \in \cV_{(x_k:N] }(A) } \cP{\zd_j}{\zd_{\pa(j)}}{} \right) &= \sum_{\zd_{(x_k: N]} \in Z_{(x_k: N]}(A)} \prob_{\Do(A)} \left[ \cV_{(x_k: N]}(A) = \zd_{(x_k: N]} | \pa (\cV_{(x_k: N]}(A)) \right]\\
  &=\prob_{\Do(A)} \left[ V_N = 1 | \pa \left( \cV_{(x_k:N] }(A) \right)\right] \leq 1.
	\end{align*}
	For all other terms, we have the following equality, 
	\begin{align*}
		\sum_{\zd\in Z_{(x_i: x_{i+1}]}(A)}& \left(\prod_{j \in \cV_{(x_i:x_{i+1}) }(A) } \cP{\zd_j}{\zd_{\pa(j)}}{} \right) 
		\\ &= \sum_{\zd_{x_{i+1}} \in \{0,1\}} \ \sum_{\zd_{(x_i: x_{i+1})} \in Z_{(x_i: x_{i+1})}(A)} \left(\prod_{j \in \cV_{(x_i:x_{i+1}) }(A) } \cP{\zd_j}{\zd_{\pa(j)}}{} \right)
		\\ &= \sum_{\zd_{x_{i+1}} \in \{0,1\}} \sum_{\zd_{(x_i: x_{i+1})} \in Z_{(x_i: x_{i+1})}(A)} \prob_{\Do(A)} \left[ \cV_{(x_i:x_{i+1}) }(A) = \zd_{(x_i: x_{i+1})} | \pa \left( \cV_{(x_i:x_{i+1}) }(A) \right)\right]
  \\ & \leq \sum_{\zd_{x_{i+1}} \in \{0,1\}} 1  \\&=  2.
	\end{align*}

Substituting in (\ref{eqn:sec}), we get 
\begin{align*}
	\sum_{\zd \in Z (A)}  \sum_{\substack{U \subseteq \cV(A) \\ |U| = k}} \left(\prod_{i \in U } \left |\Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \right |  \right) \left(\prod_{j \in \cV(A) \setminus U} \cP{\zd_j}{\zd_{\pa(j)}}{} \right) \leq \sum_{\substack{U \subseteq \cV(A) \\ |U| = k}} \left( 2 \eta\right) ^k = \binom{N}{k} \left( 2 \eta\right) ^k
\end{align*}

Therefore, the sum $\sum_{\zd \in Z(A)} \left| \mathcal{L}_\zd  \right|$ satisfies
\begin{align*}
	\sum_{\zd \in Z(A)} |\mathcal{L}_\zd | &\leq \sum_{k=2}^{N}\binom{N}{k} \left( 2 \eta\right) ^k \\
	&= \sum_{k=0}^{N}\binom{N}{k} \left( 2 \eta\right) ^k  - 2N\eta - 1 \\
	&=(1+2\eta)^N-2N\eta-1\\
	&\leq e^{2N\eta}-2N\eta -1\\
	&\leq 1 + 2N\eta + (2N\eta)^2 - 2N \eta -1 \tag{with $\eta \leq \frac{1}{2N}$}\\
	&\leq 4N^2\eta^2.
\end{align*}
The lemma stands proved. 
\end{proof}

\begin{lemma}\label{lem:h-bound}
For estimates obtained via a covering intervention set $\cI$, as in Algorithm \ref{algo: main algo fully obs setting}, the following event holds with probability at least $\left( 1-\frac{2}{T} \right)$:
    \begin{align*}
        \left| \sum_{\zd \in Z(A)}\mathcal{H}_\zd \right| \leq \sqrt{\frac{N |\cI| \log{|\cA| T}}{T}} \qquad \text{for all $A \in \cA$.}
    \end{align*}
\end{lemma}
\begin{proof}
The definition of $\mathcal{H}_\zd$ gives us
{\allowdisplaybreaks
	\begin{align*} 
		&\left| \sum_{\zd \in Z(A)}\mathcal{H}_\zd \right|\\
            &= \left|  \sum_{\zd \in Z(A)}\sum_{ i \in \cV (A)} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \prod_{ j \in \cV(A), j\neq i}  \cP{\zd_j}{\zd_{\pa(j)}}{} \right| \\
		&=  \left|  \sum_{ i \in \cV (A)} \sum_{\zd \in Z(A)} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \prod_{ j \in \cV(A), j\neq i}  \cP{\zd_j}{\zd_{\pa(j)}}{} \right| \\
		&= \left|  \sum_{ i \in \cV (A)} \sum_{\substack{\zd_{[1:i]} \in \\  Z_{[1:i]}(A)}} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \sum_{\substack{\zd_{(i: N ]} \in \\ Z_{(i:N]}(A)}} \prod_{ k \in \cV_{(i:N]}(A)}  \cP{\zd_k}{\zd_{\pa(k)}}{} \right| \\
		&= \left| \sum_{i \in \cV (A) } \sum_{\substack{\zd_{[1:i]} \in \\  Z_{[1:i]}(A)}} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \sum_{\substack{\zd_{(i: N ]} \in \\ Z_{(i:N]}(A)}} \prob_{\Do(A)} \left[\cV_{(i:N]}(A) = \zd_{(i:N ]} \mid \pa\left(\cV_{(i:N]}(A)\right)  \right] \right|\\
		&= \left| \sum_{ i \in \cV (A) } \sum_{\substack{\zd_{[1:i]} \in \\  Z_{[1:i]}(A)}} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \prob_{\Do(A)} \left[V_N = 1 \mid \pa\left(\cV_{(i:N]}(A)\right)  \right] \right|\\    
		%
		&= \left| \sum_{ i \in \cV (A) } \sum_{\zd_i \in \{0,1\}}\sum_{\substack{\zd_{[1:i)} \in \\ Z_{[1:i)}(A)}} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{}
		\prob_{\Do(A)} \left[V_N = 1 \mid \pa\left(\cV_{(i:N]}(A)\right)  \right] \right|\\
  &= \left| \sum_{ i \in \cV (A) } \sum_{\zd_i \in \{0,1\}}\sum_{\substack{\zd_{\pa(i)} \in \\ Z_{\pa(i)}(A)}} \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} \sum_{\substack{\zd_{\ac(i)} \in \\ Z_{\ac(i)}(A)}} \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \prob_{\Do(A)} \left[V_N = 1 \mid \pa\left(\cV_{(i:N]}(A)\right)  \right] \right|\\
\end{align*}
}
 Recall that $\ac(i) = [1,i) \setminus \pa(i) $ and write 
 \begin{align}
     c_i(z_i, \zd_{\pa (i)}) \coloneqq  \sum_{\substack{\zd_{\ac(i)} \in \\ Z_{\ac(i)}(A)}} \ \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \prob_{\Do(A)} \left[V_N = 1 \mid \pa\left(\cV_{(i:N]}(A)\right)  \right] \label{eqn:def-c}
 \end{align}
Also, as a shorthand for $z_i=1$ and $z_i=0$ we will write $1_i$ and $0_i$, respectively. With these notations, we have 
\begin{align*}
\left| \sum_{\zd \in Z(A)}\mathcal{H}_\zd \right| 
  &= \left| \sum_{ i \in \cV (A) } \sum_{\zd_i \in \{0,1\}} \sum_{\zd_{\pa (i)} \in Z_{\pa(i)}(A) } \Delta \cP{\zd_i}{\zd_{\pa(i)}}{} c_i(\zd_i,\zd_{\pa(i)}) \right| \\
%
		&=\left| \sum_{ i \in \cV (A) } \sum_{\zd_{\pa (i)} \in Z_{\pa(i)}(A) } \Delta \cP{1_i}{\zd_{\pa(i)}}{} \left(c_i(1_i,\zd_{\pa(i)}) - c_i(0_i,\zd_{\pa(i)}) \right)\right| \tag{since  $\Delta \cP{1_i}{\zd_{\pa(i)}}{} = -  \Delta \cP{0_i}{\zd_{\pa(i)}}{}$}
	\end{align*}

Since $\cI$ is a covering intervention set, for each pair $(i,\zd_{\pa(i)})$, there exists an intervention $I \in \cI$ such that intervening $\Do(I)$ provides a sample from the conditional probability distribution $\prob [ V_i =1 \mid \pa(V_i) = \zd_i]$. Hence, Line \ref{line:do-intervene} of the algorithm provides at least $\frac{T}{|\cI|}$ independent samples from the conditional distribution $\prob [ V_i =1 \mid \pa(V_i) = \zd_i]$. We write the $s^{th}$ sample for this conditional distribution by $Y_s(i,\zd_{\pa(i)})$. Now, we have 
\begin{align*}
	\left| \sum_{\zd \in Z(A)}\mathcal{H}_\zd \right|  = \left| \sum_{ i \in \cV (A) } \sum_{\substack{\zd_{\pa (i)} \in \\ Z_{\pa(i)}(A)}} \frac{|\cI|}{T} \left( \sum_{s=1}^{T/|\cI|} Y_s(i,\zd_{\pa(i)}) - \cP{1_i}{\zd_{\pa(i)}}{} \right)   (c_i(1_i,\zd_{\pa(i)}) - c_i(0_i,\zd_{\pa(i)}))\right|
\end{align*}
We will apply Hoeffding's inequality (Lemma \ref{lem:hoeff}) to bound the above expression. Note that in this expression, besides $Y_s(i,\zd_{\pa(i)})$-s, all the other terms are deterministic. In particular, we show in Claim \ref{lem:bound_c} (stated and proved below) that $\sum_{\zd_{\pa (i)} \in Z_{\pa(i)}(A)} (c(1_i,\zd_{\pa(i)}) - c(0_i,\zd_{\pa(i)}))^2  \leq 1$, for all $i$. Hence, for any $A \in \cA$, Lemma \ref{lem:hoeff} gives us 
\begin{align*}
	\prob \left( \left| \sum_{\zd \in Z(A)}\mathcal{H}_\zd \right| \geq \varepsilon \right) &\leq 2 \ \mathrm{exp}\left( \frac{ - T \varepsilon^2}{|\cI| \sum_{ i \in \cV (A) } \sum_{\zd_{\pa (i)} \in Z_{\pa(i)}(A) } (c_i(1_i,\zd_{\pa(i)}) - c_i(0_i,\zd_{\pa(i)}))^2} \right) \\
		&\leq 2 \ \mathrm{exp} \left( \frac{ - T \varepsilon^2}{ |\cI| \ |\cV(A)| } \right) \tag{via Claim \ref{lem:bound_c}}\\ 
		&\leq 2 \ \mathrm{exp} \left( \frac{ - T \varepsilon^2}{ |\cI| \ N } \right).
	\end{align*}
	Setting $\varepsilon = \sqrt{\frac{N \cdot |\cI| \log{(|\cA| \cdot T)}}{T}}$ and taking union bound over all $A \in \cA$, gives us the required probability bound. This completes the proof of the lemma. 
 \end{proof}
We next establish the claim used in the proof of Lemma \ref{lem:h-bound}.
\begin{claim} \label{lem:bound_c}
	\begin{align*}
		\sum_{\zd_{\pa (i)} \in Z_{\pa(i)}(A)} (c(1_i,\zd_{\pa(i)}) - c(0_i,\zd_{\pa(i)}))^2  \leq 1.
	\end{align*}
\end{claim}
\begin{proof}
The definition of $c(\zd_i, \zd_{\pa(i)})$ (see equation (\ref{eqn:def-c})) gives us 
{ \allowdisplaybreaks
	\begin{align*}
		&| c(1_i,\zd_{\pa(i)}) - c(0_i,\zd_{\pa(i)}) | 
		\\&= \biggl| \sum_{\zd \in Z_{\ac(i)}(A) } \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \prob_{\Do(A)} \left[\cV_{[i+1:N]}(A) = \zd_{[i+1:N ]} \mid \pa\left(\cV_{[1: i]}(A) \right) = (\zd_{[1:i)} \cup 1_{i} )  \right] - 
		\\ & \qquad \qquad \sum_{\zd \in Z_{\ac(i)}(A) } \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \prob_{\Do(A)} \left[\cV_{[i+1:N]}(A) = \zd_{[i+1:N ]} \mid \pa\left(\cV_{[1: i]}(A) \right)= (\zd_{[1:i)} \cup 0_{i} )  \right] \biggr|\\
        &=  \biggl| \sum_{\zd \in Z_{\ac(i)}(A) } \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{}  \biggl( \prob_{\Do(A)} \left[\cV_{[i+1:N]}(A) = \zd_{[i+1:N ]} \mid \pa (\cV_{[1: i]}(A)) = (\zd_{[1:i)} \cup 1_{i} ) \ \right] - \\ & \qquad \prob_{\Do(A)} \left[\cV_{[i+1:N]}(A) = \zd_{[i+1:N ]} \mid \pa(\cV_{[1: i]}(A) )= (\zd_{[1:i)} \cup 0_{i} )  \right] \biggr)  \biggr| \\
		&\leq   \sum_{\zd \in Z_{\ac(i)}(A) } \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \biggl| \prob_{\Do(A)} \left[\cV_{[i+1:N]}(A) = \zd_{[i+1:N ]} \mid \pa (\cV_{[1: i]}(A)) = (\zd_{[1:i)} \cup 1_{i})\right] - \\ & \qquad \qquad \prob_{\Do(A)} \left[\cV_{[i+1:N]}(A) = \zd_{[i+1:N ]} \mid \pa (\cV_{[1: i]}(A)) = (\zd_{[1:i)} \cup 0_{i} )  \right] \biggr| \\
		& \leq \sum_{\zd \in Z_{\ac(i)}(A) } \prod_{ j \in \cV_{[1:i)}(A)} \cP{\zd_j}{\zd_{\pa(j)}}{} \\
		& = \prob_{\Do(A)}\left[ \cV_{\pa(i)}(A) = \zd_{\pa(i)}\right].
	\end{align*}
}
Hence, under intervention $A \in \cA$, we have 
	\begin{align*}
		\sum_{\zd_{\pa (i)} \in Z_{\pa(i)}(A)} (c(1_i,\zd_{\pa(i)}) - c(0_i,\zd_{\pa(i)}))^2  &\leq \sum_{\zd_{\pa (i)} \in Z_{\pa(i)}(A)} |c(1_i,\zd_{\pa(i)}) - c(0_i,\zd_{\pa(i)})|\\
		&\leq \sum_{\zd_{\pa (i)} \in Z_{\pa(i)}(A)} \prob_{\Do(A)}\left[ \cV_{\pa(i)}(A) = \zd_{\pa(i)}\right] \\
		&\leq 1.
	\end{align*}
This completes the proof of the claim.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm: main theorem full obs}]
Lemma \ref{lem:covers} implies that, with probability at least $\left(1 - \frac{1}{T}\right)$, the set $\cI$ obtained in Line \ref{line:construct-cover} of Algorithm \ref{algo: main algo fully obs setting} is indeed a covering intervention set. We combine this guarantee with Lemmas \ref{lem:l-bound} and \ref{lem:h-bound}. In particular, with probability at least $\left(1- \frac{5}{T}\right)$, we have, for all $A \in \cA$:
\begin{align*}
  \left|\mu(A) - \muh(A)\right|   &= \left|\sum_{\zd \in Z(A)} \left( \mathcal{H}_\zd + \mathcal{L}_\zd \right) \right|\\
        &\leq \sqrt{\frac{N |\cI| \log{|\cA| T}}{T}} + \frac{4 N^2 |\cI| (d+\log{(NT)})}{T}\\
        &\leq 2\sqrt{\frac{N |\cI| \log{|\cA| T}}{T}} \tag{For $T \gtrsim  N^3$}
\end{align*}
Let $A_T \in \cA$ be the intervention returned by Algorithm \ref{algo: main algo fully obs setting} (after $T$ rounds of interventions), i.e., $A_T = \argmax_{A\in \cA} \ \muh(A)$. In addition, $A^* = \argmax_{A \in \cA} \ \mu(A)$ be the optimal intervention. Hence, with probability at least $\left(1-\frac{5}{T} \right)$, we have 
    \begin{align}
        \mu(A^*)- \mu(A_T) \leq 4  \sqrt{\frac{N |\cI| \log{|\cA| T}}{T}} 
    \end{align}
This guarantee gives us the desired upper bound on the simple regret, $R_T$, of Algorithm \ref{algo: main algo fully obs setting}: 
\begin{align*}
    R_T = \E \left[ \mu(A^*)- \mu(A_T) \right] &\leq  \left(4  \sqrt{\frac{N |\cI| \log{|\cA| T}}{T}}\right) \left(1-\frac{5}{T}\right) + \frac{5}{T} \ \ \leq \ 5 \sqrt{\frac{N |\cI| \log{|\cA| T}}{T}}.
\end{align*}
Since the size of the covering intervention set satisfies $|\cI| = 3d \cdot  2^d (\log N +2d + \log T )$ (see Lemma \ref{lem:covers}), we also have the following explicit form of the simple regret bound
\begin{align*}
	R_T = {O} \left( \sqrt{ \frac{N \ d 2^d \ \log |\cA| }{T} } \log T  \right).
\end{align*}
The theorem stands proved. 
\end{proof}
